A practical model-based segmentation approach for improved activation detection in single-subject functional Magnetic Resonance Imaging studies

Functional Magnetic Resonance Imaging (fMRI) maps cerebral activation in response to stimuli but this activation is often difficult to detect, especially in low-signal contexts and single-subject studies. Accurate activation detection can be guided by the fact that very few voxels are, in reality, truly activated and that these voxels are spatially localized, but it is challenging to incorporate both these facts. We address these twin challenges to single-subject and low-signal fMRI by developing a computationally feasible and methodologically sound model-based approach, implemented in the R package MixfMRI, that bounds the a priori expected proportion of activated voxels while also incorporating spatial context. An added benefit of our methodology is the ability to distinguish voxels and regions having different intensities of activation. Our suggested approach is evaluated in realistic two- and three-dimensional simulation experiments as well as on multiple real-world datasets. Finally, the value of our suggested approach in low-signal and single-subject fMRI studies is illustrated on a sports imagination experiment that is often used to detect awareness and improve treatment in patients in persistent vegetative state (PVS). Our ability to reliably distinguish activation in this experiment potentially opens the door to the adoption of fMRI as a clinical tool for the improved treatment and therapy of PVS survivors and other patients.

==> e02-table.tex <==
%\subsection{Summary Tables of Main Simulation Results}
%\renewcommand{\arraystretch}{0.9}
\setlength{\tabcolsep}{1pt}
\begin{table*}[ht]
\caption{ Performance, on simulations with the three phantoms of all methods including
  ours with $K$ selected 
  using BIC and ICL-BIC followed respectively by P2 and P3 merging,
  and with and without spatial context. For each 
  setting and method, we report the median Jaccard index with the
  interquartile range of the Jaccard indices in parenthesis.
}
%\input{plots_fdr_ss/fdr_tables_weighted/simu_fdr_JI_0.99.txt}
{\fontsize{8.75}{8.2}\selectfont
  \input{tables_s/newtable.txt}}
\label{tab:newtable}
\end{table*}
%\FloatBarrier
\begin{comment}
\FloatBarrier
\begin{table}[ht]
\centering
\label{tab:simu_JI_I_975}
\caption{Performance on simulations done with  $\hat{\pi}_0 \geq
  0.975$ $(\delta = 0.975)$ set for our method, using the 

  as in Table~\ref{tab:simu_JI_I_99}
          proposed methods. $\hat{\pi}_0 \geq 0.975$ $(\delta = 0.975)$
          is set for this table.
          The P3 merging procedure is used.
}
%\input{plots_fdr_ss/fdr_tables_weighted/simu_fdr_JI_0.975.txt}
\input{tables_s/simu_fdr_JI_0.975.txt}
\end{table}
\FloatBarrier




\begin{table}[ht]
\centering
\label{tab:simu_JI_I_95}
\caption{ The Jaccard index based on merged $K$ for main results of all
          proposed methods. $\hat{\pi}_0 \geq 0.95$ $(\delta = 0.95)$
          is set for this table.
          The P3 merging procedure is used.
}
%\input{plots_fdr_ss/fdr_tables_weighted/simu_fdr_JI_0.95.txt}
\input{tables_s/simu_fdr_JI_0.95.txt}
\end{table}
\FloatBarrier

\end{comment}
